Robotic Long-Horizon Manipulation with Progressive In-Context Code Generation and Episodic Feedback

Robotic long-horizon manipulation requires robots to compose perception, reasoning, and action over extended task sequences, yet existing language-conditioned frameworks often rely on dense step-wise feedback, learned action policies, or unstructured prompting, which limits robustness and generalization. We propose DAHLIA, a data-agnostic code-generation framework that treats long-horizon manipulation as episodic task planning and evaluation. DAHLIA uses progressively organized in-context examples with chain-of-thought reasoning to guide an LLM in synthesizing executable code plans from language instructions. To improve robustness under partial observability, a VLM-based reporter evaluates task outcomes only after each execution episode and provides structured feedback for replanning, avoiding the overhead of per-step inference. Experiments on LoHoRavens, CALVIN, Franka Kitchen, and real-world manipulation tasks show that DAHLIA achieves strong performance on over 30 long-horizon tasks and improves generalization to unseen scenarios, including cluttered scenes and occluded objects.

==> imgs/00_overview.tex <==
\begin{figure}[t!]
    \centering
    \resizebox{.5\textwidth}{!}{
    \begin{tikzpicture}
        \fill[white, rounded corners=4pt, shading=axis, left color=ffgreen_pv!50, right color=fforange_pv!50]
            (-3.5cm,-1cm) -- (3.5cm,-1cm) -- (3.5cm,-2.8cm) -- (-3.5cm,-2.8cm) -- cycle;
        \fill[white] (0,0) -- (3.6cm, 0) -- (3.6cm, -2.9cm) -- (0, -2.9cm) --cycle;
        \fill[white, rounded corners=4pt, shading=axis, left color=ffgreen_pv!50, right color=fforange_pv!50]
            (-3.5cm, 1cm) -- (3.5cm, 1cm) -- (3.5cm, 2.8cm) -- (-3.5cm, 2.8cm) -- cycle;
        \fill[white] (0,0) -- (-3.6cm, 0) -- (-3.6cm, 2.9cm) -- (0, 2.9cm) --cycle;
        
        \shade[left color=ffgreen_pv!50, right color=fforange_pv!50] (0,0) circle (2.8cm);
        \node[circle, draw=white, fill=none, line width=4pt, minimum size=4cm](line)at(0,0){};
        \draw[draw=white, line width=3pt, rounded corners=2pt] (0, -1.95cm) -- (0.5cm, -2.4cm) -- (0, -2.85cm);
        \draw[draw=white, line width=3pt, rounded corners=2pt] (0, 1.95cm) -- (-0.5cm, 2.4cm) -- (0, 2.85cm);
        \path[decorate,decoration={text along path, text={|\footnotesize\sf\bfseries\color{white}|Planner Tunnel},text align=center, raise=-0.2cm}] (180:2.5cm) arc (180:120:2.5cm);
        \path[decorate,decoration={text along path, text={|\footnotesize\sf\bfseries\color{white}|Reporter Tunnel},text align=center, raise=-0.2cm}] (0:2.5cm) arc (0:-60:2.5cm);
        \node[]at(1.8,2.3){\footnotesize \textcolor{white}{\textsf{Closed-loop Feedback}}};
        \node[]at(-1.8,-2.2){\footnotesize \textcolor{white}{\textsf{Chain-of-Thought}}};
        \node[]at(-1.8,-2.6){\footnotesize \textcolor{white}{\textsf{Temporal Abstraction}}};
        \clip (0,0) circle (2cm) node (scene) {\includegraphics[width=4cm]{imgs/realworld_cover.pdf}};
        
        
    \end{tikzpicture}
    }
    \vskip -0.05in
    \caption{Overview of our proposed framework. The dual-tunnel structure generates executable task plans and enables closed-loop feedback. By incorporating temporal abstraction and CoT-based guidance, our approach substantially enhances agent performance in both simulation and real-world long-horizon manipulation tasks.}
    \label{fig:Overview}
\vskip -0.15in
\end{figure}

==> imgs/01_framework.tex <==
%
%
\begin{figure*}[ht!]
% \vskip -0.2in
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tikzpicture}
        % BG
        \shade[left color=ffgreendark_pv!40, right color=fforange_pv!40] (15,-5) circle (5.75cm);
        \node[circle, fill=white, minimum size=10cm] at (15,-5){};
        \fill[ffgreendark_pv!50, rounded corners=4pt, shading=axis, left color=ffgreendark_pv!50, right color=ffgreendark_pv!20]
            (5,0) -- (10,0) -- (15,-5) -- (10,-10) -- (5, -10) -- cycle;
        \fill[fforange_pv!50, rounded corners=4pt, shading=axis, left color=fforange_pv!20, right color=fforange_pv!50]
            (15, -5) -- (20,0) -- (25,0) -- (25,-10) -- (20,-10) -- cycle;
        \node[circle, draw=none, fill=white, line width=1pt, minimum size=9cm](white_circle)at(15,-5){};
        \shade[left color=ffgreen_pv!50, right color=fforange_pv!50] (15,-5) circle (4.25cm);
        \node[circle, fill=white, minimum size=8cm] (env_bg) at (15,-5){};
        
        % Env
        \node[circle, fill=none, minimum size=1cm](env)at(15,-5){\includegraphics[width=8cm]{imgs/env.png}};
        \node[circle, fill=white] (tasks) at (15,-5){\textbf{\textsf{Tasks}}};
        % \node[circle, draw=gray, minimum size=1.1cm, line width=2pt] at (15,-5){};

        % user
        \fill[fflightgreen!60, rounded corners=3pt, shading=axis, left color=fflightgreen!20, right color=fflightgreen!60]
            (0,0) -- (4,0) -- (4.5,-0.5) -- (4.5,-2.5) -- (0.5, -2.5) -- (0, -2) -- cycle;
        \fill[fflightgreen!20, rounded corners=3pt]
            (0.3,-3.3) -- (4.75,-3.3) -- (4.75,-10) -- (0.3, -10) -- cycle;
        % \node[inner sep=-1pt, circle, draw=fflightgreen, fill=white, line width=1pt, label={[label distance=-0.45cm]-90:\small \textsf{User}}](miyabi)at(0,-1){\includegraphics[width=1.5cm]{imgs/miyabi.png}};
        % \node[inner sep=-1pt, circle, draw=fflightgreen, fill=none, line width=1pt, minimum size=2.2cm](line)at(0,-1){};
        \node[inner sep=-1pt, circle, draw=fflightgreen, fill=white, line width=1pt, label={[label distance=-0.55cm]-90:\small \textsf{User}}](miyabi)at(0,-1){\includegraphics[width=1.5cm]{imgs/user.png}};
        \node[inner sep=-1pt, circle, draw=fflightgreen, fill=none, line width=1pt, minimum size=2.3cm](line)at(0,-1){};
        
        
        \node[text width=3cm]at([xshift=1.7cm, yshift=-0.2cm]miyabi.east){\large \textsf{Can you use blocks to build a 2*2*2 cube in the zone?}};
        \node[]at([xshift=2cm, yshift=-1cm]miyabi.south){\large \textcolor{fflightgreen}{\textbf{\textsf{Prompted with:}}}};
        
        \node[rectangle, draw=none, fill=fflightgreen!60, rounded corners=3pt, minimum width=4cm, minimum height=1cm, text width=3.2cm, align=left](prompt1)at([xshift=2.5cm, yshift=-2cm]miyabi.south){\large \textsf{1. Available APIs}};
        \node[rectangle, draw=none, fill=fflightgreen!60, rounded corners=3pt, minimum width=4cm, minimum height=1cm, text width=3.2cm, align=left](prompt2)at([yshift=-1cm]prompt1.south){\large \textsf{2. Coordinates}};
        \node[rectangle, draw=none, fill=fflightgreen!60, rounded corners=3pt, minimum width=4cm, minimum height=1cm, text width=3.2cm, align=left](prompt3)at([yshift=-1cm]prompt2.south){\large \textsf{3. Rules}};
        \node[rectangle, draw=none, fill=fflightgreen!60, rounded corners=3pt, minimum width=4cm, minimum height=1cm, text width=3.2cm, align=left](prompt4)at([yshift=-1cm]prompt3.south){\large \textsf{4. Example plan}};
        \node[]at([yshift=-0.5cm]prompt4.south){\large \textcolor{fflightgreen}{\textbf{\textsf{Chain-of-Thought}}}};

        \draw[-{Circle}, draw=fflightgreen!80, line width=3pt, rounded corners=1pt] (miyabi.south) |- ([xshift=7pt]prompt1.west);
        \draw[-{Circle}, draw=fflightgreen!80, line width=3pt, rounded corners=1pt] (miyabi.south) |- ([xshift=7pt]prompt2.west);
        \draw[-{Circle}, draw=fflightgreen!80, line width=3pt, rounded corners=1pt] (miyabi.south) |- ([xshift=7pt]prompt3.west);
        \draw[-{Circle}, draw=fflightgreen!80, line width=3pt, rounded corners=1pt] (miyabi.south) |- ([xshift=7pt]prompt4.west);

        % planner
        \node[rectangle, draw=none, fill=ffdarkgreen!40, rounded corners=3pt, minimum width=4cm, minimum height=1.25cm](planner_bg)at([xshift=6.7cm, yshift=-1.2cm]miyabi.east){};
        \draw[->, draw=ffdarkgreen, line width=2pt, rounded corners=1pt] ([xshift=-0.2cm]planner_bg.south east) to[out=-60, in=60] ++ (0, -2.4cm);
        \node[rectangle, draw=none, fill=ffdarkgreen!30, rounded corners=3pt, minimum width=4cm, minimum height=1.25cm](planner)at([xshift=6.5cm, yshift=-1cm]miyabi.east){\Large \textsf{Planners}};
        \node[rectangle, draw=none, fill=ffdarkgreen!30, rounded corners=3pt, minimum width=4cm, minimum height=1.25cm](tasks)at([yshift=-1.3cm]planner.south){\Large \textsf{Task plan}};
        \node[rectangle, draw=none, fill=ffdarkgreen!30, rounded corners=3pt, minimum width=4cm, minimum height=1.25cm](lmp)at([yshift=-1.3cm]tasks.south){\Large \textsf{LMPs/APIs}};
        \node[rectangle, draw=none, fill=ffdarkgreen!50, rounded corners=3pt, minimum width=4cm, minimum height=1.25cm](primitives_bg0)at([xshift=0.4cm, yshift=-1.7cm]lmp.south){};
        \node[rectangle, draw=none, fill=ffdarkgreen!40, rounded corners=3pt, minimum width=4cm, minimum height=1.25cm](primitives_bg1)at([xshift=0.2cm, yshift=-1.5cm]lmp.south){};
        \node[rectangle, draw=none, fill=ffdarkgreen!30, rounded corners=3pt, minimum width=4cm, minimum height=1.25cm](primitives)at([yshift=-1.3cm]lmp.south){\Large \textsf{Primitives}};
        \node[](dots)at([yshift=-0.5cm]primitives_bg1.south){\Large \textsf{\textbf{\dots}}};

        \draw[->, draw=ffdarkgreen, line width=2pt, rounded corners=1pt] (planner.south) -- (tasks.north);
        \draw[->, draw=ffdarkgreen, line width=2pt, rounded corners=1pt] (tasks.south) -- (lmp.north);
        \draw[->, draw=ffdarkgreen, line width=2pt, rounded corners=1pt] (lmp.south) -- (primitives.north);
        % \draw[->, draw=ffdarkgreen!70, line width=2pt, rounded corners=2pt] ([yshift=-0.2cm]planner_bg.east) -| ++ (0.5cm, -0.5cm) |- (lmp.east);

        % reporter
        \node[rectangle, draw=none, fill=fforange_pv!20, rounded corners=3pt, minimum width=4cm, minimum height=1.25cm](reporter)at([xshift=21.5cm, yshift=-1cm]miyabi.east){\Large \textsf{Reporter}};
        \node[rectangle, draw=none, fill=fforange_pv!20, rounded corners=3pt, minimum width=4cm, minimum height=1.25cm](eval)at([yshift=-1.3cm]reporter.south){\Large \textsf{Evaluation}};
        \node[rectangle, draw=none, fill=fforange_pv!20, rounded corners=3pt, minimum width=4cm, minimum height=1.25cm](lmp2)at([yshift=-1.3cm]eval.south){\Large \textsf{LMPs/APIs}};
        \node[rectangle, draw=none, fill=fforange_pv!20, rounded corners=3pt, minimum width=4cm, minimum height=1.25cm](obs)at([yshift=-1.3cm]lmp2.south){\Large \textsf{Observation}};

        \draw[->, draw=fforange_pv, line width=2pt, rounded corners=1pt] (obs.north) -- (lmp2.south);
        \draw[->, draw=fforange_pv, line width=2pt, rounded corners=1pt] (lmp2.north) -- (eval.south);
        \draw[->, draw=fforange_pv, line width=2pt, rounded corners=1pt] (eval.north) -- (reporter.south);

        % bent text and arrows
        \begin{scope}[shift={(15,-5)}] % Move the center to (15, -5)
            \path[decorate, decoration={text along path, text={|\sf|A 2*2*2 cube is stacked in the zone, task complete.}, text align=center}] (135:5.25) arc (135:45:5.25);
            \path[decorate,decoration={text along path, text={|\sf|Is task ``cube stack'' succeed?}, text align=center}] (225:5.5) arc (225:315:5.5);
        \end{scope}

        \draw[-{Triangle Cap []. Fast Triangle[]}, draw=fflightgreen!80, line width=8pt, rounded corners=1pt] ([xshift=-1cm]planner.west) -- (planner.west);
        \draw[-{Triangle Cap []. Fast Triangle[]}, draw=ffdarkgreen!80, line width=8pt, rounded corners=1pt] ([xshift=1.7cm, yshift=0.8cm]planner.east) to[out=225, in=0] (planner.east);
        \draw[-{Triangle Cap []. Fast Triangle[]}, draw=ffdarkgreen!80, line width=8pt, rounded corners=1pt] (env_bg) to[out=143, in=0] (planner.east);
        \draw[-{Triangle Cap []. Fast Triangle[]}, draw=ffdarkgreen!80, line width=8pt, rounded corners=1pt] (primitives.east) to[out=0, in=210] (env_bg);
        \draw[-{Triangle Cap []. Fast Triangle[]}, draw=ffdarkgreen!80, line width=8pt, rounded corners=1pt] (primitives.east) to[out=0, in=135] ([xshift=1.75cm, yshift=-1cm]primitives.east);
        \draw[-{Triangle Cap []. Fast Triangle[]}, draw=fforange_pv!80, line width=8pt, rounded corners=1pt] (env_bg) to[out=325, in=180] (obs.west);
        \draw[-{Triangle Cap []. Fast Triangle[]}, draw=fforange_pv!80, line width=8pt, rounded corners=1pt] ([xshift=-1.75cm, yshift=-1cm]obs.west) to[out=45, in=180] (obs.west);
        \draw[-{Triangle Cap []. Fast Triangle[]}, draw=fforange_pv!80, line width=8pt, rounded corners=1pt] (reporter.west) to[out=180, in=-45] ([xshift=-1.7cm, yshift=0.8cm]reporter.west);
        \node[draw=none, fill=none]at(6.5,-0.5){\LARGE \textsf{\textbf{\textcolor{white}{PLANNER}}}};
        \node[draw=none, fill=none]at(23.25,-0.5){\LARGE \textsf{\textbf{\textcolor{white}{REPORTER}}}};
    \end{tikzpicture}
    }
    \vskip -0.1in
    \caption{Framework of DAHLIA. Our framework utilizes a dual-tunnel structure to implement a planner-reporter closed-loop feedback mechanism for various long-horizon manipulation tasks. The planner, powered by LLMs, converts high-level language instructions and initial state into task plans, leveraging available LMPs/APIs to generate multi-step motion primitives with the idea of temporal abstraction. The reporter, powered by a VLM, evaluates task outcomes using visual observations and provides feedback to the planner, enabling dynamic re-planning and robust performance in unstructured environments.}
    \vskip -0.2in
    \label{fig:framework}
\end{figure*}




==> imgs/02_task_snapshot.tex <==
\begin{figure*}[ht!]
\vskip -0.2in
\centering
\resizebox{\textwidth}{!}{
\begin{tikzpicture}
    % First row of images
    \node[rectangle, clip, rounded corners=2pt, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(A)}}}] (img1) at (0,0) {\includegraphics[width=0.18\textwidth]{imgs/all_on_zone.jpg}};
    % "Stack all blocks in the indigo zone."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img1, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(B)}}}] (img2) {\includegraphics[width=0.18\textwidth]{imgs/block_same_size.jpg}};
    % "Stack blocks of the same size in the yellow zone and the other yellow zone respectively."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img2, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(C)}}}] (img3) {\includegraphics[width=0.18\textwidth]{imgs/block_same_color.jpg}};
    % "Stack all the blocks of the same color together in the same colored zone."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img3, , label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(D)}}}] (img4) {\includegraphics[width=0.18\textwidth]{imgs/block_color_and_size.jpg}};
    % "Stack only the bigger blocks of cool color in the yellow zone."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img4, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(E)}}}] (img5) {\includegraphics[width=0.18\textwidth]{imgs/relative_pos_and_color.jpg}};
    % "Stack all the blocks, which are to the rear of the indigo block with front-back distance larger than 0.05 unit, in the silver zone."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img5, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(F)}}}] (img6) {\includegraphics[width=0.18\textwidth]{imgs/move_absolu.jpg}};
    % "Move all the blocks in the top-left area to bottom-left area."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img6, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(G)}}}] (img7) {\includegraphics[width=0.18\textwidth]{imgs/move_absolu_size.jpg}};
    % "Move all the smaller blocks in the bottom-right area to bottom-left area."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img7, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(H)}}}] (img8) {\includegraphics[width=0.18\textwidth]{imgs/matching_bowl.jpg}};
    % "Put the blocks in the bowls with matching colors."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img8, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(I)}}}] (img9) {\includegraphics[width=0.18\textwidth]{imgs/mismatching_bowl.jpg}};
    % "Put the blocks in the bowls with mismatching colors."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img9, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(J)}}}] (img10) {\includegraphics[width=0.18\textwidth]{imgs/alternate_color.jpg}};
    % "Stack blocks with alternate colors on the indigo zone, starting with the cyan color."
    
    % second row of images
    \node[rectangle, rounded corners=2pt, clip, below=0.2cm of img1, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(G1)}}}] (img11) {\includegraphics[width=0.18\textwidth]{imgs/build_pyramid.jpg}};
    % "Construct a 9-4-1 rectangular pyramid structure in the zone using 14 blocks of the same color."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img11, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(G2)}}}] (img12) {\includegraphics[width=0.18\textwidth]{imgs/build_cube.jpg}};
    % "Construct a 2*2*2 cube structure in the zone using 8 blocks of the same color."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img12, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(G3)}}}] (img13) {\includegraphics[width=0.18\textwidth]{imgs/circle_with_blocks.jpg}};
    % "Construct a circle with suitable radius with alternating red and blue blocks in the zone."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img13, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(G4)}}}] (img14) {\includegraphics[width=0.18\textwidth]{imgs/circle_ball_middle.jpg}};
    % "Construct a circle with suitable radius with alternating purple and pink blocks around the ball."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img14, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(G5)}}}] (img15) {\includegraphics[width=0.18\textwidth]{imgs/concentric_circles.jpg}};
    % "Construct two concentric circles in the zone using 7 violet and 11 brown blocks."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img15, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(G6)}}}] (img16) {\includegraphics[width=0.18\textwidth]{imgs/divide_blocks.jpg}};
    % "Divide the blocks into groups of 3 and stack each group in a different zone."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img16, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(G7)}}}] (img17) {\includegraphics[width=0.18\textwidth]{imgs/max_odd_number.jpg}};
    % "Place the maximal odd number of blocks of the same color in each correspondingly colored zone."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img17, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(G8)}}}] (img18) {\includegraphics[width=0.18\textwidth]{imgs/stack_most_color_blocks.jpg}};
    % "Stack blocks of the same color that has the largest quantity in the zone."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img18, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(G9)}}}] (img19) {\includegraphics[width=0.18\textwidth]{imgs/zone_bisector.jpg}};
    % "Arrange all blocks on the zone bisector line evenly."
    
    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img19, label={[label distance=-0.2cm]-90:\small \textbf{\textsf{(G10)}}}] (img20) {\includegraphics[width=0.18\textwidth]{imgs/different_fixture.jpg}};
    % "Fill in all L-shaped fixtures with blocks of different colors."

    \node[below right] at([yshift=-0.2cm]img11.south west) (table) {
    % \rowcolors{0}{white}{gray!30}
    \begin{tabular}{c m{14.25cm} | c m{14.25cm}}
        \toprule
        \rowcolor{nature_tab_gray1}
        \textbf{Label} & \textbf{Instructions of Original Tasks} & \textbf{Label} & \textbf{Instructions of Generated Tasks} \\
        \midrule
        A & "Stack all blocks in the [COLOR] zone." & G1 & "Construct a 9-4-1 rectangular pyramid structure in the zone using 14 blocks of the same color." \\
        \rowcolor{nature_tab_gray2}
        \midrule
        B & "Stack blocks of the same size in the [COLOR1] zone and [COLOR2] zone respectively." & G2 & "Construct a 2*2*2 cube structure in the zone using 8 blocks of the same color." \\
        \midrule
        C & "Stack all the blocks of the same color together in the same colored zone." & G3 & "Construct a circle with suitable radius with alternating [COLOR1] and [COLOR2] blocks in the zone." \\
        \midrule
        \rowcolor{nature_tab_gray2}
        D & "Stack only the [SIZE] blocks of [COLOR\_TYPE] color in the [COLOR] zone." & G4 & "Construct a circle with suitable radius with alternating [COLOR1] and [COLOR2] blocks around the ball." \\
        \midrule
        E & "Stack all the blocks, which are to the [REL\_POS] of the [COLOR1] block with [POS\_TYPE] distance larger than 0.05 unit, in the [COLOR2] zone." & G5 & "Construct two concentric circles in the zone using [NUM] [COLOR1] and [NUM + 4] [COLOR2] blocks." \\
        \midrule
        \rowcolor{nature_tab_gray2}
        F & "Move all the blocks in the [POS1] area to [POS2] area." & G6 & "Divide the blocks into groups of [NUM] and stack each group (also including the group with block number less than [NUM]) in a different zone." \\
        \midrule
        G & "Move all the [SIZE] blocks in the [POS1] area to [POS2] area." & G7 & "Place the maximal odd number of blocks of the same color in each correspondingly colored zone." \\
        \rowcolor{nature_tab_gray2}
        \midrule
        H & "Put the blocks in the bowls with matching colors." & G8 & "Stack blocks of the same color that has the largest quantity in the zone." \\
        \midrule
        I & "Put the blocks in the bowls with mismatching colors." & G9 & "Arrange all blocks on the zone bisector line between two symmetrically placed zones evenly on the tabletop, and the gap between two adjacent blocks' edges should be near the block size, and the line connecting the center of the zones also bisects these blocks." \\
        \midrule
        \rowcolor{nature_tab_gray2}
        J & "Stack blocks with alternate colors on the [COLOR1] zone, starting with the [COLOR2] color." & G10 & "Each L-shaped fixture can hold three blocks, suppose the block size is (a,a,a), then in fixture's local coordinate system, the three places that can hold blocks are [(0,0,0),(a,0,0),(0,a,0)]. Fill in all the fixtures which have random position and rotation with blocks, and make sure in the end in every fixture there are three blocks with different colors." \\
        \bottomrule
    \end{tabular}
};
\end{tikzpicture}
}
\vskip -0.05in
\caption{Completion snapshots of LoHoRavens Benchmark and generated tasks. The first row shows tasks from LoHoRavens, and the second row demonstrates generated tasks. The table shows the corresponding task instructions.}
\label{fig:snapshots}
\vskip -0.25in
\end{figure*}



==> imgs/03_calvin_kitchen_snapshots.tex <==
\begin{figure}[htb!]
\vskip -0.05in
\centering
\resizebox{.485\textwidth}{!}{
\begin{tikzpicture}
% First row of images
    \node[rectangle, clip, rounded corners=2pt, label={[label distance=-0.6cm]-90:\small \textbf{\textsf{lift block}}}] (img1) at (0,0) {\includegraphics[width=0.18\textwidth]{imgs/calvin_lift.png}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img1, label={[label distance=-0.6cm]-90:\small \textbf{\textsf{rotate block}}}] (img2) {\includegraphics[width=0.18\textwidth]{imgs/calvin_rotate.png}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img2, label={[label distance=-0.6cm]-90:\small \textbf{\textsf{turn on switch}}}] (img3) {\includegraphics[width=0.18\textwidth]{imgs/calvin_switch.png}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img3, label={[label distance=-0.6cm]-90:\small \textbf{\textsf{open slide door}}}] (img4) {\includegraphics[width=0.18\textwidth]{imgs/calvin_slide.png}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img4, label={[label distance=-0.6cm]-90:\small \textbf{\textsf{open drawer}}}] (img5) {\includegraphics[width=0.18\textwidth]{imgs/calvin_drawer.png}};

    % second row
    \node[rectangle, clip, rounded corners=2pt, below=0.1cm of img1, label={[label distance=-0.6cm]-90:\small \textbf{\textsf{\textcolor{white}{microwave}}}}] (img6) {\includegraphics[width=0.18\textwidth]{imgs/kitchen_microwave.png}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img6, label={[label distance=-0.6cm]-90:\small \textbf{\textsf{\textcolor{white}{kettle}}}}] (img7) {\includegraphics[width=0.18\textwidth]{imgs/kitchen_kettle.png}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img7, label={[label distance=-0.6cm]-90:\small \textbf{\textsf{\textcolor{white}{burner}}}}] (img8) {\includegraphics[width=0.18\textwidth]{imgs/kitchen_burner.png}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img8, label={[label distance=-0.6cm]-90:\small \textbf{\textsf{\textcolor{white}{slide cabinet}}}}] (img9) {\includegraphics[width=0.18\textwidth]{imgs/kitchen_slide_cabinet.png}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img9, label={[label distance=-0.6cm]-90:\small \textbf{\textsf{\textcolor{white}{hinge cabinet}}}}] (img10) {\includegraphics[width=0.18\textwidth]{imgs/kitchen_hinge_cabinet.png}};


\end{tikzpicture}

}
\vskip -0.05in
\caption{Completion state snapshots of CALVIN and Franka Kitchen benchmarks. The first row shows illustrations from CALVIN, and the second row demonstrates images from Franka Kitchen.}
\label{fig:calvin_kitchen_snapshots}
\vskip -0.05in
\end{figure}

==> imgs/04_realworld_demo.tex <==
\begin{figure}[ht!]
% \vskip -0.05in
\centering
\resizebox{.485\textwidth}{!}{
\begin{tikzpicture}
% First row of images
    \node[rectangle, clip, rounded corners=2pt,] (img1) at (0,0) {\includegraphics[width=0.18\textwidth]{imgs/task1_1.pdf}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img1,] (img2) {\includegraphics[width=0.18\textwidth]{imgs/task1_2.pdf}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img2, ] (img3) {\includegraphics[width=0.18\textwidth]{imgs/task1_3.pdf}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img3, ] (img4) {\includegraphics[width=0.18\textwidth]{imgs/task1_4.pdf}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img4,] (img5) {\includegraphics[width=0.18\textwidth]{imgs/task1_5.pdf}};

    % second row
    \node[rectangle, clip, rounded corners=2pt, below=0.1cm of img1,] (img6) {\includegraphics[width=0.18\textwidth]{imgs/task2_1.pdf}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img6, ] (img7) {\includegraphics[width=0.18\textwidth]{imgs/task2_2.pdf}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img7, ] (img8) {\includegraphics[width=0.18\textwidth]{imgs/task2_3.pdf}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img8, ] (img9) {\includegraphics[width=0.18\textwidth]{imgs/task2_4.pdf}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img9, ] (img10) {\includegraphics[width=0.18\textwidth]{imgs/task2_5.pdf}};

    % third row
    \node[rectangle, clip, rounded corners=2pt, below=0.1cm of img6, ] (img11) {\includegraphics[width=0.18\textwidth]{imgs/task3_1.pdf}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img11, ] (img12) {\includegraphics[width=0.18\textwidth]{imgs/task3_2.pdf}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img12,] (img13) {\includegraphics[width=0.18\textwidth]{imgs/task3_3.pdf}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img13, ] (img14) {\includegraphics[width=0.18\textwidth]{imgs/task3_4.pdf}};

    \node[rectangle, rounded corners=2pt, clip, right=0.005cm of img14,] (img15) {\includegraphics[width=0.18\textwidth]{imgs/task3_5.pdf}};


\end{tikzpicture}

}
\vskip -0.05in
\caption{Snapshots of real-world demonstrations. Pick all fruits and place them on the plate (1st row). Stack blocks in a pyramid shape (2nd row). Make the coffee from the coffee machine (3rd row).}
\label{fig:realworld}
\vskip -0.1in
\end{figure}
